BiaScope: Visual Unfairness Diagnosis for Graph Embeddings

The issue of bias (i.e., systematic unfairness) in machine learning models has recently attracted the attention of both researchers and practitioners. For the graph mining community in particular, an important goal toward algorithmic fairness is to detect and mitigate bias incorporated into graph embeddings since they are commonly used in human-centered applications, e.g., social-media recommendations. However, simple analytical methods for detecting bias typically involve aggregate statistics which do not reveal the sources of unfairness. Instead, visual methods can provide a holistic fairness characterization of graph embeddings and help uncover the causes of observed bias. In this work, we present BiaScope, an interactive visualization tool that supports end-to-end visual unfairness diagnosis for graph embeddings. The tool is the product of a design study in collaboration with domain experts. It allows the user to (i) visually compare two embeddings with respect to fairness, (ii) locate nodes or graph communities that are unfairly embedded, and (iii) understand the source of bias by interactively linking the relevant embedding subspace with the corresponding graph topology. Experts' feedback confirms that our tool is effective at detecting and diagnosing unfairness. Thus, we envision our tool both as a companion for researchers in designing their algorithms as well as a guide for practitioners who use off-the-shelf graph embeddings.

==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/additional_packages.tex <==
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{hyperref}
\usepackage{xspace}


==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/tex_input/data-preprocessing.tex <==
\subsection{Data Management}\label{sec:preprocessing}
Due to the size of the networks that were considered, several performance challenges needed to be addressed in the development process. In this section, we provide an overview of how these were approached.

As previously outlined, in order to improve network visibility, we filter out visually non-salient edges. Specifically, we only display edges in the top 10 percent of length. Filtering allows us to save on browser memory, as the number of edges far exceeds the number of nodes. At the same time, by inspecting the networks we found that the bottom 90 percent of shortest edges were often not visible, so filtering offers large performance increases while preserving important visual information, e.g., intra-community connectivity.

In terms of preprocessing, both the projection of the embeddings, as well as group and individual fairness scores were calculated offline in order to obtain an additional performance speedup. For the later, this involves generating for every network the corresponding score for each node id and possible configuration. Configuration options consist of the number of hops from the focal node for the individual fairness notion, while for the group fairness, the value of $k$ as well as the chosen sensitive attribute (in our case gender) and value.

Finally, the pre-computed network information is accessed only once when the webpage is initially loaded and stored in memory, in order to avoid redundant server access.

==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/tex_input/expert-review.tex <==
\subsection{Expert Feedback}\label{sec:expert_review}


In order to evaluate our tool, we conducted feedback interviews with our two collaborators and two additional experts, who are active researchers interested in graph embeddings, also affiliated with Northeastern’s Network Science Institute. We conducted four individual interviews, during which each participant was able to interact with the tool through the webpage on their own system. We simultaneously observed their interaction with the tool, which was captured on video for further analysis. For all interviews we followed the same steps: First, we asked for the participant's consent to video recording. Second, we briefly discussed the tasks our tool is designed to support. Third, we provided an \textit{interactive walk-through} of the tool by asking the participant to locate certain views and perform concrete tasks. The goal of this step was to help the participants familiarize themselves with the UI. Next, we encouraged the participant to follow a \textit{usage scenario} similar to the one presented in Section \ref{sec:usage_scenario}. During this step we provided loose guidance by setting open-ended goals and we encouraged the participant to freely accomplish them using the tool. Lastly, we collected verbal feedback using the following questions:
\begin{itemize}
    \item[\textbf{Q1}] In your view, how well are the domain tasks supported?
    \item[\textbf{Q2}] How would you perform these tasks without the tool? Do you see value in our tool?
    \item[\textbf{Q3}] How would you use our tool in your research/development process?
    \item[\textbf{Q4}] What limitations do you identify?
\end{itemize}
%We note that participants tended to also express their thoughts and offer feedback during the interactive walk-through and the usage scenario, as they were interacting with the tool. 
Following the interview sessions, we collected additional quantitative feedback from the experts using a System Usability Scale (SUS) \cite{sus_1}. In what follows, we summarize the key takeaways from the feedback. 

\paragraph{Effectiveness and Usability.} 
% Q1:
% All agree: Task support is really good. 
% Tina: Summary statistics are well selected

% Q2: 
% All say or describe that they would do the same thing we did! They point out it would be time saving
% Brennan: Would use the tool, since “I don’t want to implement any of this by myself”. Says it’s immediately useful in a time saving way.
% Zohair: saves time

% Exact quotes
% BK (51:55): something that goes a long way in terms of what you've done is like I don't want to implement any of these things [by myself]

During the interactive walk-through, we observed that all the participants were able to quickly perform the tasks with little to no assistance. Regarding explicit verbal feedback, all experts agreed that \biascope effectively supports the described domain tasks (\textbf{Q1}). Additionally, all participants described, while three explicitly said, that they would follow the same process in order to thoroughly analyse unfairness of a graph embedding (\textbf{Q2}). Most participants pointed out that without \biascope this analysis would be tedious and prone to errors. One participant mentioned that \biascope would save them time and a different one said: ``something that goes a long way in terms of what you have done is I do not want to implement any of these things [by myself]. ... at the very basic level you have just reallocated a lot of work... [Since there are no other tools like this one on the market], this is immediately useful in a very time saving way.''. 

% Q3: 
% Zohair (26:30): sanity check
% For people who aren't really fairness focused, this would [enable] a nice quick sanity check.
% 
% Tina
% (25:01) I think, so I would do something similar to what you guys have done um and I don't know again how hard, this is this is this is amazing to me like you guys put a lot of work into this, which is fantastic. But like I would have it, be more hierarchical as opposed to like when I diagnose it and I pick a node I only see the node and it's neighborhood where, for example, I could select a group, maybe if I bring this back here and share my screen again i'm.
% 
% Tina: Tool is great to interrogate the data before using it in the context of an ML model, which is a very important task
% (27:20) yeah I would use it like as as visualization so basically just like interrogating the data right so interrogating the data is a very important thing to do right as opposed to just feeding it into your machine learning system and then hoping for the best.
% 
% Ayan: could also see it used to explain concrete downstream tasks in the context of explainable embeddings. 
% (28:12) ... I would definitely use this tool for understanding explainability and interpretability of embeddings ... my major use would be like explaining some of the down stream task results or predictions that i'm getting 
% 
% Brennan: also as a good teaching device. He believes that web pages with these characteristics (in particular with interactivity) are positive in general in this sense.
% BK (54:30) It is very, it is very good teaching tool in general I think like web based things that let you interact with networks, change the game when it comes to learning about networks.

Regarding the potential role of \biascope within our participants' research process (\textbf{Q3}), the feedback validated the tool's effectiveness while additionally providing new perspectives. Two of the experts agreed that the tool would facilitate the evaluation of their graph embedding algorithms with respect to fairness. More specifically, they mentioned the following: ``For people who aren't really fairness focused, this would [enable] a nice quick sanity check.'' and ``I would use it as a visual tool to interrogate the data, [which is] a very important thing to do, as opposed to just feeding it into your machine learning system and then hoping for the best.'' The other two experts pointed out they could further utilize our tool to facilitate their work in explainable machine learning or for pedagogical purposes:  ``... I would definitely use this tool for understanding explainability and interpretability of embeddings ... my major use would be like explaining some of the down stream task results or predictions'', ``It is a very good teaching tool, in general I think web based [tools] that let you interact with networks, change the game when it comes to learning about networks.''. 


\paragraph{Limitations.}
% most participants: need to be able to upload their own embedding (csv)
% Brennan: would like to export the table and other info
% agreed: need to fix the scale of the embedding to convey understanding of what is the magnitude of "far" in the overall embedding.
% Zohair: also add a simple example network (typical topology) beyond the benchmarks, so people can understand the fairness definitions
% common suggestion (Zohair, Ayan, Brennan): add info (on-demand) about fairness definitions on the page

The experts agreed on the importance of an ``import" feature, which would allow the user to upload and diagnose their own embedding algorithm. One of the experts additionally suggested an ``export" functionality. The implementation of an “import” feature is included as future work in Section \ref{sec:limitations_futurework}. Moreover, some experts pointed out that the Diagnose View should include an indication of the scale regarding the projected embeddings, in order to clearly convey the magnitude of distances observed in the local embedding subspace. We addressed this limitation with the addition of the context legend, as discussed in Section \ref{sec:design}. One of the experts expressed the interesting idea to augment our network options with certain simple synthetic networks representing typical graph topologies, e.g., star, which could enlighten the user with respect to the nature of different fairness notions. Finally, adding on-demand information about the selected fairness notion definition was a frequent suggestion among participants.


\paragraph{System Usability Scale.} 
We requested our experts to fill a System Usability Scale (SUS) \cite{sus_1, brooke2013sus}, a standard simple ten-item scale giving a global view of subjective assessments of the usability of a system. Based on the responses, we derive the corresponding SUS scores, which have a range of 0 to 100. Regarding scores assessment, \cite{bangor_etal} proposed an adjective value scale for SUS scores. According to this scale, scores in the range 72.5-84.9 are associated with a good usability and above 85 represent an excellent one. Based on the collected SUS scores, we obtained a mean value of $83.125$. This implies, per the aforementioned scale, that \biascope's usability was perceived as good, close to excellent by the interviewed experts.

% We calculated an average value from the ratings of the 9 participants with a result of 75 (SD = 9.52), with median of 80. Hence, we received reasonable or good ratings for usability from our study participants.

%----
% From Glyphboard:
% over 80 represent a good or excellent usability. Between 60 and 80, usability can be regarded between bad and good.
%----

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%          Adjective & Mean SUS Score \\
%          \hline
%          Worst Imaginable & 12.5\\
%          Poor & 35.7\\
%          OK & 50.9\\
%          Good & 71.4\\
%          Excellent & 85.5\\
%          Best Imaginable & 90.9 \\
%     \end{tabular}
%     \caption{Adjective Ratings for SUS scores presented in \cite{bangor_etal}.}
%     \label{tab:sus_adj_scores}
% \end{table}



==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/tex_input/graph-datasets.tex <==
\begin{table}[ht]
    \centering
    \begin{minipage}{\linewidth}
    \centering
    \begin{tabular}{| l | l | r | r | r |}\hline
         \textbf{Graph} & \textbf{Type} & $n$ & $m$ & $C$\\ \hline
         Wikipedia \cite{node2vec}& Language & 4.8K & 185K & 1\\
         Facebook \cite{snapnets}& Social & 4.0K & 88K& 1\\
         PPI \cite{node2vec}& Biological & 3.9K & 77K & 35\\
        %  ca-HepTh & Citation & 9.9K & 26K & 429 \\
         LastFM \cite{snapnets}& Social & 7.6K & 28K & 1 \\
        %  Books \footnote{\url{http://www-personal.umich.edu/~mejn/netdata/}} & E-commerce & 105 & 441 & 1 \\
        %  NS \cite{netscience-data} & Co-author & 1.5K & 2.7K & 268 \\ \hline
        %  AS & Internet & 23K & 48K & 1\\ 
        \hline
    \end{tabular}
    \end{minipage}
    \caption{We test our design on four real-world graphs spanning multiple domains. All of the networks are thousands of nodes. Above $n$ is the number of nodes, $m$ is the number of edges, and $C$ is the number of connected components.}
    \label{tab:snap_datasets}
\end{table}

==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/tex_input/task-table-short.tex <==
\begin{table*}[ht]
\centering
\label{tab:tasks}
\begin{tabular}{|p{0.2\linewidth}|p{0.3\linewidth}|p{0.07\linewidth}|p{0.07\linewidth}|p{0.08\linewidth}||p{0.08\linewidth}|}
% \toprule
\hline

\multicolumn{2}{|c|}{\textbf{Domain Tasks}} & \multicolumn{4}{|c|}{\textbf{Abstract Tasks}}\\ \hline
Task & Example and Description & High & Mid & Low & Graph-Specific \\\hline

\textbf{Statistical Summary} & Degree distribution, avg. degree, clustering coefficient, triangle count & Derive & Explore & Characterize Distribution & Overview \\\hline

\textbf{Embedding Comparison \textit{w.r.t.} Fairness} & Compare two embeddings w.r.t. a fairness score per node, per topological community or for the whole graph & Present & Explore & Correlate & Overview \\\hline

\textbf{Unfairness Diagnostics} & For a given embedding, find which nodes contribute to unfairness and why & Discover & Locate & Find Anomalies & Attribute-based: On the Nodes\\\hline

\end{tabular}
\caption{\biascope is designed to support the domain tasks described in the table, which facilitate our complete unfairness diagnosis workflow for graph embeddings. For each domain task on the left, we provide a detailed explanation and then we list the high, mid, and low level abstract tasks \cite{munzner2014visualization, amar2005low} along with the graph-specific abstract task \cite{lee2006task}.}
\end{table*}

==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/tex_input/task-table.tex <==
\begin{table*}[ht]
\centering
\caption{Based on our interview with Professor Tina Eliassi-Rad we extracted the tasks described in the table. For each domain task on the left, we provide an example and then we list the high, mid, and low level abstract tasks \cite{munzner2014visualization, amar2005low} along with the graph-specific abstract task \cite{lee2006task}.  The domain tasks are listed in order of priority. }
\label{tab:tasks_full}
\begin{tabular}{|p{0.2\linewidth}|p{0.3\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}||p{0.1\linewidth}|}
\toprule
\multicolumn{2}{|c|}{\textbf{Domain Tasks}} & \multicolumn{4}{|c|}{\textbf{Abstract Tasks}}\\ \hline
Task & Example and Description & High & Mid & Low & Graph-Specific \\\hline

\textbf{Statistical Summary} & Degree distribution, avg. degree, clustering coefficient, triangle count & Derive & Explore & Characterize Distribution & Overview \\\hline

\textbf{Embedding Comparison \textit{w.r.t.} Fairness} & Compare two embeddings w.r.t. a fairness score per node, per topological community or for the whole graph & Present & Explore & Correlate & Overview \\\hline

\textbf{Unfairness Diagnostics} & For a given embedding, find which nodes contribute to unfairness and why & Discover & Locate & Find Anomalies & Attribute-based: On the Nodes\\\hline
\\\hline
Community Detection & Separating the graph into groups & Derive & Explore & Cluster & Topology: Find Clusters \\\hline

Community Labeling & Labeling detected communities (e.g., by political party) & Annotate & Browse & Compute Derived Value & Attribute-based: On the Nodes \\\hline

Fairness Definitions Comparison & Individual vs. Group fairness: determining the impact of the fairness definition on the embedding location for a set of nodes. & Present & Browse & Correlate & Attribute-based: On the Nodes\\\hline

Set Hyperparameter Values for Fairness Definition & Determining the impact of hyperparameters on the fairness score for a set of nodes, for a given fairness definition. & Discover & Explore & Correlate & Attribute-based: On the Nodes\\\hline

Check for Representation Stability & Re-running the algorithm multiple times. & Present & Lookup & Cluster & Overview\\\hline

Disentangling Features from Topology & In a social network: visualize info from a users profile vs unified info from their friend group & Discover & Locate & Correlate & Attribute-based: On the Nodes\\\hline

Filter Graph & Filter nodes/edges e.g. filter all of the female nodes in a social network & Discover & Locate & Filter & Attribute-based: On the Nodes \\\hline

Manipulate Graph & Adding edges between nodes with common neighbors (triadic closure) & Derive & Lookup & Compute Derived Value  &  Topology: Accessibility\\\hline

Tracking Dynamic Processes & Message Passing (spread of information e.g. influence maximization and spread of disease) & Discover & Locate & Correlate & Overview\\\hline

Outlier Detection & Fraud detection & Discover & Locate & Find Anomalies & Overview\\\hline

\bottomrule
\end{tabular}
\end{table*}

==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/tex_input/usability-testing.tex <==
\subsection{Usability Testing}\label{sec:usability_testing}

During the development of our tool we performed an informal usability testing session with 15 Computer Science graduate student as our participants. The goal of this study was to qualitatively evaluate the effectiveness of our visual encodings for the target tasks as well as the usability of the interactivity elements. 

The study confirmed that there exist certain technical barriers for non-specialist users, which is understandable since our design was targeted to experts. However, we still took action to clarify certain components, for example we implemented user-friendly tooltips for explanations and definitions of technical terms. Additionally, the study was particularly revealing with respect to color encodings and color perception. More specifically, it indicted that the users tend to associate dark colors with more unfairness and red colors are semantically associated with pathological attributes, which in our case correspond to biased embeddings. Finally, the study reassured us that the implemented interactivity significantly empowers the user to investigate causes of bias and successfully complete unfairness diagnostics. 

==> 2022-VDS@VIS-BiaScope_ Visual Unfairness Diagnosis for Graph Embeddings/tex_input/usage-scenario.tex <==
\subsection{Usage Scenario}\label{sec:usage_scenario}
To illustrate the design in action, we will walk through a case study using the Facebook network, which represents the social network friendships of over four thousand users. We begin with an overview of the network via the statistical summary shown in Figure \ref{fig:statistical-summary}. The table on the left informs the user that the Facebook graph is sparse and highly clustered. Further, the degree distribution shows that almost all users in the network have fewer than 200 friends.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/SS.png}
    \caption{The statistical summary for the Facebook network helps the user to characterize the data before analyzing its fairness scores. The table on the left states that the network is sparse and highly clustered while the degree distribution shows that almost all users in the network have fewer than 200 friends.}
    \label{fig:statistical-summary}
\end{figure}

Proceeding further into the \textit{Overview}, the user can browse a side-by-side comparison of the fairness scores for two sets of embeddings. Figure \ref{fig:teaser}B shows the scores for Node2Vec on the left and then HGCN on the right for the Facebook network. This visual provides two takeaways. First, the Node2Vec embeddings are overall more fair than the HGCN embeddings, as indicated by the lighter coloring. Second, the unfairness for HGCN is concentrated in select communities. Without the visualization, a purely statistical analysis would resort to aggregate values which do not account for heterogeneity. 

Moving into the drill down portion of the tasks, we can now use the \textit{Diagnose View} to better understand why certain nodes are scored as unfair. For instance, Figure \ref{fig:inform-diagnose} shows the diagnostic results for the Facebook Node2Vec embeddings using the individual fairness notion. The local neighborhood (ego network) shows that the focal node, in red, is part of two communities of friends. Further, the projected embeddings show that the two communities of friends are embedded far from each other. Hence, the focal node is scored as unfair because it is far from its neighbor communities in embedding space. This mapping between neighbors and embeddings can be verified with brushing and linking (Figure \ref{fig:diagnose_view_1}). 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/inform-diagnose-new.png}
    \caption{Moving into the drill-down tasks, the above figure provides the diagnostics results for the Facebook network's Node2Vec embeddings where fairness is defined with the InFoRM notion of individual fairness. The ego network on the left shows the target node is part of two communities, as linked on the right hand side, these communities are themselves embedded far apart. Thus, the diagnostics results show that under InFoRM bridge nodes between communities may be embedded unfairly. }
    \label{fig:inform-diagnose}
\end{figure}

Finally, the user can also drill-down and diagnose the group fairness scores as well. Figure \ref{fig:fairwalk-diagnose} shows the Facebook Node2Vec embeddings evaluated based on the group fairness notion. Now, the focal node together with the induced subgraph (top-$k$ recommended nodes) is plotted in the rightmost chart. The subgraph shows that the target node's recommendations are mostly of gender 0, encoded in yellow, which is a form of homophily. Further, these nodes are embedded close to the target node in the embedding space. This is a form of group unfairness because if we train a model to recommend friends based on these embeddings, the model would perpetuate homophily for this node and recommend nodes of the same gender. 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/fairwalk-diagnose-new.png}
    \caption{The diagnostics results for group fairness show that the given node from the Facebook network is unfair because many of its recommended nodes are also of the same gender value, encoded in yellow. The focal node and the induced subgraph given by the top-$k$ recommended nodes are plotted, together with the corresponding embeddings. The design layout is similar to the individual fairness diagnostics but the node colors now represent the sensitive attribute, which is the most important attribute for group fairness.}
    \label{fig:fairwalk-diagnose}
\end{figure}



==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tex_input/task-table.tex <==
\begin{table*}[ht]
\centering
\caption{Based on our interview with Professor Tina Eliassi-Rad we extracted the tasks described in the table. For each domain task on the left, we provide an example and then we list the high, mid, and low level abstract tasks \cite{munzner2014visualization, amar2005low} along with the graph-specific abstract task \cite{lee2006task}.  The domain tasks are listed in order of priority. }
\label{tab:tasks_full}
\begin{tabular}{|p{0.2\linewidth}|p{0.3\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}||p{0.1\linewidth}|}
\toprule
\multicolumn{2}{|c|}{\textbf{Domain Tasks}} & \multicolumn{4}{|c|}{\textbf{Abstract Tasks}}\\ \hline
Task & Example and Description & High & Mid & Low & Graph-Specific \\\hline

\textbf{Statistical Summary} & Degree distribution, avg. degree, clustering coefficient, triangle count & Derive & Explore & Characterize Distribution & Overview \\\hline

\textbf{Embedding Comparison \textit{w.r.t.} Fairness} & Compare two embeddings w.r.t. a fairness score per node, per topological community or for the whole graph & Present & Explore & Correlate & Overview \\\hline

\textbf{Unfairness Diagnostics} & For a given embedding, find which nodes contribute to unfairness and why & Discover & Locate & Find Anomalies & Attribute-based: On the Nodes\\\hline
\\\hline
Community Detection & Separating the graph into groups & Derive & Explore & Cluster & Topology: Find Clusters \\\hline

Community Labeling & Labeling detected communities (e.g., by political party) & Annotate & Browse & Compute Derived Value & Attribute-based: On the Nodes \\\hline

Fairness Definitions Comparison & Individual vs. Group fairness: determining the impact of the fairness definition on the embedding location for a set of nodes. & Present & Browse & Correlate & Attribute-based: On the Nodes\\\hline

Set Hyperparameter Values for Fairness Definition & Determining the impact of hyperparameters on the fairness score for a set of nodes, for a given fairness definition. & Discover & Explore & Correlate & Attribute-based: On the Nodes\\\hline

Check for Representation Stability & Re-running the algorithm multiple times. & Present & Lookup & Cluster & Overview\\\hline

Disentangling Features from Topology & In a social network: visualize info from a users profile vs unified info from their friend group & Discover & Locate & Correlate & Attribute-based: On the Nodes\\\hline

Filter Graph & Filter nodes/edges e.g. filter all of the female nodes in a social network & Discover & Locate & Filter & Attribute-based: On the Nodes \\\hline

Manipulate Graph & Adding edges between nodes with common neighbors (triadic closure) & Derive & Lookup & Compute Derived Value  &  Topology: Accessibility\\\hline

Tracking Dynamic Processes & Message Passing (spread of information e.g. influence maximization and spread of disease) & Discover & Locate & Correlate & Overview\\\hline

Outlier Detection & Fraud detection & Discover & Locate & Find Anomalies & Overview\\\hline

\bottomrule
\end{tabular}
\end{table*}

==> tex_input/usability-testing.tex <==
\subsection{Usability Testing}\label{sec:usability_testing}

During the development of our tool we performed an informal usability testing session with 15 Computer Science graduate student as our participants. The goal of this study was to qualitatively evaluate the effectiveness of our visual encodings for the target tasks as well as the usability of the interactivity elements. 

The study confirmed that there exist certain technical barriers for non-specialist users, which is understandable since our design was targeted to experts. However, we still took action to clarify certain components, for example we implemented user-friendly tooltips for explanations and definitions of technical terms. Additionally, the study was particularly revealing with respect to color encodings and color perception. More specifically, it indicted that the users tend to associate dark colors with more unfairness and red colors are semantically associated with pathological attributes, which in our case correspond to biased embeddings. Finally, the study reassured us that the implemented interactivity significantly empowers the user to investigate causes of bias and successfully complete unfairness diagnostics. 
